Debugging WebAssembly? Put some Whamm on it!

Debugging and monitoring programs are integral to engineering and deploying software. Dynamic analyses monitor applications through source code or IR injection, machine code or bytecode rewriting, and virtual machine or direct hardware support. While these techniques are viable within their respective domains, common tooling across techniques is rare, leading to fragmentation of skills, duplicated efforts, and inconsistent feature support. We address this problem in the WebAssembly ecosystem with Whamm, a declarative instrumentation DSL for WebAssembly that abstracts above the instrumentation strategy, leveraging bytecode rewriting and engine support as available. Whamm solves three problems: 1) tooling fragmentation, 2) prohibitive instrumentation overhead of general-purpose frameworks, and 3) tedium of tailoring low-level high-performance mechanisms. Whamm provides fully-programmable instrumentation with declarative match rules, static and dynamic predication, automatic state reporting, and user library support, while achieving high performance through compiler and engine optimizations. At the back end, Whamm provides instrumentation to a Wasm engine as Wasm code, reusing existing engine optimizations and unlocking new ones, most notably intrinsification, to minimize overhead. In particular, explicitly requesting program state in match rules, rather than reflection, enables the engine to efficiently bundle arguments and even inline compiled probe logic. Whamm streamlines the tooling effort, as its bytecode-rewriting target can run instrumented programs everywhere, lowering fragmentation and advancing the state of the art for engine support. We evaluate Whamm with case studies of non-trivial monitors and show it is expressive, powerful, and efficient.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

#all:  ${PDF} ALLSAMPLES
#
#
#%.pdf:  %.dtx   $(PACKAGE).cls
#	pdflatex $<
#	- bibtex $*
#	pdflatex $<
#	- makeindex -s gind.ist -o $*.ind $*.idx
#	- makeindex -s gglo.ist -o $*.gls $*.glo
#	pdflatex $<
#	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
#	do pdflatex $<; done

all:  paper.pdf

view: paper.pdf
	open paper.pdf &

paper.pdf: paper.tex intro.tex authors.tex whamm-instr.tex optimizations.tex implementation.tex evaluation.tex related-work.tex conclusion.tex data-availability.tex $(PACKAGE).cls figures/*.pdf paper.bib
	pdflatex $<
	bibtex paper
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.08.  Section titles are in lowercase now.
	       Documentation updates.

Version 2.07.  Corrected typo in TELO eISSN.

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> artifact.tex <==
\section{The Artifact}

More information can be found here (at least for 2024): \url{https://2024.splashcon.org/track/splash-2024-oopsla-artifacts#Call-for-Artifacts}

\subsection{Introduction}

In the \textbf{Introduction}, briefly explain the purpose of the artifact and how it supports the paper.
We recommend listing all claims in the paper and stating whether or not each is supported.
For supported claims, say how the artifact provides support.
For unsupported claims, explain why they are omitted.

\todo{Add artifact introduction content.}

\subsection{Hardware Dependencies}

In the \textbf{Hardware Dependencies} section, describe the hardware required to evaluate the artifact.
If the artifact requires specific hardware (e.g., many cores, disk space, GPUs, specific processors), please provide instructions on how to gain access to the hardware.
Keep in mind that reviewers must remain anonymous.

\todo{Add artifact Hardware Dependencies content.}

\subsection{Getting Started Guide}

In the \textbf{Getting Started Guide}, give instructions for setup and basic testing.
List any software requirements and/or passwords needed to access the artifact.
The instructions should take roughly 30 minutes to complete.
Reviewers will follow the guide during an initial kick-the-tires phase and report issues as they arise.

The Getting Started Guide should be as simple as possible, and yet it should stress the key elements of your artifact.
Anyone who has followed the Getting Started Guide should have no technical difficulties with the rest of your artifact.

\todo{Add artifact Getting Started Guide content.}

\subsection{Step-by-Step Instructions}

In the \textbf{Step by Step Instructions}, explain how to reproduce any experiments or other activities that support the conclusions in your paper.
Write this for readers who have a deep interest in your work and are studying it to improve it or compare against it.
If your artifact runs for more than a few minutes, point this out, note how long it is expected to run (roughly) and explain how to run it on smaller inputs.
Reviewers may choose to run on smaller inputs or larger inputs depending on available resources.

Be sure to explain the expected outputs produced by the Step by Step Instructions.
State where to find the outputs and how to interpret them relative to the paper.
If there are any expected warnings or error messages, explain those as well.
Ideally, artifacts should include sample outputs and logs for comparison.

\todo{Add artifact Step-by-Step Instructions content.}

\subsection{Reusability Guide}

In the \textbf{Reusability Guide}, explain which parts of your artifact constitute the core pieces which should be evaluated for reusability.
Explain how to adapt the artifact to new inputs or new use cases.
Provide instructions for how to find/generate/read documentation about the core artifact.
Articulate any limitations to the artifact’s reusability.

If the Artifact Overview is written in a language like Markdown or TeX, then authors are encouraged to upload the rendered output to HotCRP and include the source files in the artifact.

\todo{Add artifact Reusability Guide content.}

%\section{Overview of the Artifact}
%
%The overview should consist of five parts:
%\begin{itemize}
%    \item a brief Introduction,
%    \item a Hardware Dependencies section,
%    \item a Getting Started Guide, and
%    \item Step-by-Step Instructions for how you propose to evaluate the functionality of your artifact (with appropriate connections to the relevant sections of your paper).
%    \item a Reusability Guide for how you propose to evaluate the reusability of your artifact.
%\end{itemize}
%
%In the \textbf{Introduction}, briefly explain the purpose of the artifact and how it supports the paper.
%We recommend listing all claims in the paper and stating whether or not each is supported.
%For supported claims, say how the artifact provides support.
%For unsupported claims, explain why they are omitted.
%
%In the \textbf{Hardware Dependencies} section, describe the hardware required to evaluate the artifact.
%If the artifact requires specific hardware (e.g., many cores, disk space, GPUs, specific processors), please provide instructions on how to gain access to the hardware.
%Keep in mind that reviewers must remain anonymous.
%
%In the \textbf{Getting Started Guide}, give instructions for setup and basic testing.
%List any software requirements and/or passwords needed to access the artifact.
%The instructions should take roughly 30 minutes to complete.
%Reviewers will follow the guide during an initial kick-the-tires phase and report issues as they arise.
%
%The Getting Started Guide should be as simple as possible, and yet it should stress the key elements of your artifact.
%Anyone who has followed the Getting Started Guide should have no technical difficulties with the rest of your artifact.
%
%In the \textbf{Step by Step Instructions}, explain how to reproduce any experiments or other activities that support the conclusions in your paper.
%Write this for readers who have a deep interest in your work and are studying it to improve it or compare against it.
%If your artifact runs for more than a few minutes, point this out, note how long it is expected to run (roughly) and explain how to run it on smaller inputs.
%Reviewers may choose to run on smaller inputs or larger inputs depending on available resources.
%
%Be sure to explain the expected outputs produced by the Step by Step Instructions.
%State where to find the outputs and how to interpret them relative to the paper.
%If there are any expected warnings or error messages, explain those as well.
%Ideally, artifacts should include sample outputs and logs for comparison.
%
%In the \textbf{Reusability Guide}, explain which parts of your artifact constitute the core pieces which should be evaluated for reusability.
%Explain how to adapt the artifact to new inputs or new use cases.
%Provide instructions for how to find/generate/read documentation about the core artifact.
%Articulate any limitations to the artifact’s reusability.
%
%If the Artifact Overview is written in a language like Markdown or TeX, then authors are encouraged to upload the rendered output to HotCRP and include the source files in the artifact.
%
%\section{Packaging the Artifact}
%
%When packaging your artifact, please keep in mind:
%\begin{itemize}
%    \item how accessible you are making your artifact to other researchers
%    \item the fact that the AEC members have a limited time in which to make an assessment of each artifact.
%\end{itemize}
%
%A good way to package artifacts is as a virtual machine (VM).
%VMs give an easily reproducible environment that is somewhat resistant to bit rot.
%They also give reviewers confidence that errors or other problems cannot cause harm to their machines.
%We recommend that you provide VMs built for both x86 and ARM so reviewers can run the VM on whichever architecture matches their personal computer.
%
%Source code artifacts should use Docker or another build tool to manage all compilation and dependencies.
%This improves the odds that the reviewers will be able to quickly and painlessly install the artifact — without getting lost in environment issues (e.g. what Python do I need?!).
%
%Mechanized proof artifacts should follow the guidelines on this page: Proof Artifacts (accessed 2023-10-02).
%Be sure to explain how the mechanization encodes concepts and theorems from the paper.
%In our experience, it is difficult for a mechanized artifact to satisfy the requirements for Functional alone without also being Reusable because documentation is crucial for understanding whether the artifact faithfully supports the paper.
%
%Submit your artifact as a single archive file and use the naming convention <paper #>.<suffix>, where the appropriate suffix is used for the given archive format.
%sPlease use a widely available compressed archive format such as ZIP (.zip), tar and gzip (.tgz), or tar and bzip2 (.tbz2).
%Please use open formats for documents (such as .txt, .html, and .pdf).
%
%Based on the outcome of the previous editions (2019 AEC, 2020 AEC, 2021 AEC, 2023 AEC), the strongest recommendation we can give for ensuring quality packaging is to test your own directions on a fresh machine (or VM), following exactly the directions you have prepared.
%
%While publicly available artifacts are often easier to review, and considered to be in the best interest of open science, artifacts are not required to be public and/or open source.
%The submission site will ask whether the artifact is private.
%Artifact reviewers will be instructed that such artifacts are for use only for artifact evaluation, that submitted versions of artifacts may not be made public by reviewers, and that copies of artifacts must not be kept beyond the review period.
